Resolved Stars in M83 based on HST/WFC3 Early Release Science Observations

We present a multi-wavelength photometric study of individual stars in M83 based on observations taken as part of the WFC3 Early Release Science (ERS) program. The central region of M83 has been imaged in seven broad-band filters to obtain multi-wavelength coverage from the near-UV to near-IR. We use four filters- F336W, F438W, F555W, and F814W-to measure the UBVI photometric colors and intrinsic luminosity for ~10,000 stars. These measurements are used to determine the recent (< 1 Gyr) star formation history of M83. We selected 50 regions in the spiral arm and the inter-arm area of M83 and categorize them based on their H? morphology. To determine ages of stars in each region, the color-magnitude diagrams (CMD) and the color-color diagrams were used with the Padova isochrones with a metallicity of Z=0.03 (1.5 Z{\odot}). We correct the foreground and internal extinction of individual stars using the reddening-free Q parameter and improve our age estimates of stars from the isochrone fitting on the CMDs. Comparisons of stellar ages and cluster ages based on both their H? morphology and their spectral energy distribution (SED) fitting were made and show fairly good correlations. We also find that the regions with ages determined younger than 10 Myr are located preferentially along the active star-forming regions on the spiral arm.

==> up2010_refs_m83.tex <==
\begin{thebibliography}{}

\bibitem[Chandar \etal, 2010]{chandar10} Chandar, R., Whitmore, B.~C., Kim, H., \etal, 2010, ApJ, 719, 966\smallskip

\bibitem[Dopita \etal, 2010]{dopita10} Dopita, M.~A., \etal, 2010, ApJ, 710, 964\smallskip

\bibitem[Koekemoer \etal, 2002]{koekemoer02} Koekemoer, A.~M., Fruchter, A.~S., Hook, R.~N., \& Hack, W., 2002, in The 2002 \hst ~Calibration Workshop: Hubble after the Installation of the ACS and the NICMOS Cooling System, ed. S. Arribas, A. Koekemoer, \& B. Whitmore (Baltimore, MD: STScI), 337\smallskip

\bibitem[Massey \etal, 1995]{massey95} Massey, P., Armandroff, T.~E., Pyke, R., Patel, K., \& Wilson, C.~D., 1995, AJ, 110, 2715\smallskip

\bibitem[Schechter \etal, 1993]{schechter93} Schechter, P.~L., Mateo, M., \& Saha, A., 1993, PASP, 105, 1342\smallskip

\bibitem[Schlegel \etal, 1998]{schlegel98} Schlegel, D.~J., Finkbeiner, D.~P., \& Davis, M., 1998, ApJ, 500, 525\smallskip 

\bibitem[Thim \etal, 2003]{thim03} Thim, F., Tammann, G.~A., Saha, A., Dolphin, A., Sandage, A., Tolstoy, E., \& Labhardt, L., 2003, ApJ, 590, 256\smallskip

\bibitem[Toomre, 1977]{toomre77} Toomre, A., 1977, AR\&A, 15, 437\smallskip

\bibitem[Whitmore \etal, 2010]{whitmore10} Whitmore, B.~C., Chandar, R., Kim, H., \etal, 2011, in prepress\smallskip

\end{thebibliography}

